Learning Payment-Free Resource Allocation Mechanisms

We consider the design of mechanisms that allocate limited resources among self-interested agents using neural networks. Unlike the recent works that leverage machine learning for revenue maximization in auctions, we consider welfare maximization as the key objective in the payment-free setting. Without payment exchange, it is unclear how we can align agents' incentives to achieve the desired objectives of truthfulness and social welfare simultaneously, without resorting to approximations. Our work makes novel contributions by designing an approximate mechanism that desirably trade-off social welfare with truthfulness. Specifically, (i) we contribute a new end-to-end neural network architecture, ExS-Net, that accommodates the idea of "money-burning" for mechanism design without payments; (ii)~we provide a generalization bound that guarantees the mechanism performance when trained under finite samples; and (iii) we provide an experimental demonstration of the merits of the proposed mechanism.

==> whiteboard.tex <==

\begin{mechanism*}{Proportional Fairness}
\vspace{-12pt}
\begin{align}
f^{PF}(v,x,b)=& \argmin_{a\in\mathbb{R}^{NM}}-{\textstyle\sum}_{i=1}^{N}w_i\log(a_i^{\top}v_i)\label{def:PF}\\
& \hspace{-10pt} \text{s.t.} \ 0\leq a\leq x,\ {\textstyle\sum}_{i=1}^{N}a_{i,m}\leq b_m,\,\,\!\!\forall m.\notag
\end{align}
% refer to this mechanism \ref{mec:PF}
%\vspace{-25pt}
\end{mechanism*}

With $D=\vct{1}_{N}^{\top}\otimes I_{M\times M}\in\mathbb{R}^{M\times NM}$, the last inequality of \eqref{def:PF} can be expressed in the matrix form $D a\leq b$.


% Exploitability can characterize equilibria in games \cite{goktas2022exploitability}. 
It is important to note that the PF mechanism is not IC, i.e., it has nonzero exploitability. This fact motivates us to develop ways to ensure it is approximately so by trading off NSW. 
\begin{figure}
  %\vspace{-10pt}
  \centering
  \includegraphics[width=.7\linewidth]{Figures/exploitability_2x2.png}
  \vspace{-10pt}
  \caption{Exploitability of PF and learned ExPF-Net mechanisms (dashed lines indicate the utility of agent 1 under truthful report). Agent $1$ increases its utility by misreporting.\looseness=-1}
  \vspace{-10pt}
  \label{fig:exploitability_2x2}
\end{figure}

We develop two new learning-based mechanisms for resource allocation, both of which can be regarded as the composition of a function approximation (in this work, we use a feed-forward neural network) and a specific-purpose activation function. The first mechanism, ExPF-Net, is a regularized variant of the PF mechanism that diverts allocation from what the agents would like to receive when they misreport to their largest advantage. The second mechanism, ExS-Net, employs parameter augmentation via an artificial agent and provides lower complexity alternative at the cost of a minor reduction in NSW. A schematic representation of both mechanisms is presented in Figure~\ref{fig:flow}.

\begin{figure}[h]
  \centering
  \vspace{-8pt}
  \includegraphics[width=.85\linewidth]{Figures/flow.png}
  \vspace{-8pt}
  \caption{ExPF-Net and ExS-Net Pipeline, the key difference being the innovation in the output layers/activation.} 
  \vspace{-10pt}
  \label{fig:flow}
\end{figure}

%\vspace{-5pt}
\subsection{Robustness to Distribution Mismatch}\label{sec:distribution_shifts}
%\vspace{-5pt}
Let $\omega^{\star}(F)$ denote an optimizer of \eqref{eq:ExPF_obj_ERM} under samples $\{(v^l,x^l,b^l)\}_l$ drawn from the distribution $F$. 
 Next, we establish that the performance of $f_{\omega^{\star}(F')}$ on samples from  distribution $F$ when trained on samples from a different distribution $F'$ in terms of the worst-case exploitability is controlled by the degree of mismatch.
%
%
% , we show that a mechanism trained under one distribution can still work well under a slightly shifted distribution during inference. Later in Sec.~\ref{sec:exp:dist_mismatch}, we will confirm through numerical simulations that the learned mechanism is indeed robust to training and inference distribution mismatch.
\begin{thm}\label{lem:dist_mismatch}
    Given mechanism $f\in\{f_\omega^{ExPF},f_\omega^{ExS}\}$ with parameter $\omega$ which is $\epsilon$-incentive compatible over distribution $F'$, we have for any $i=1,\cdots,N$
    \vspace{-2pt}
    \begin{align*}
        E_{(v,x,b)\sim F}[\exploitability_i(f,v,x,b)]\leq\epsilon + 2M\,\overline{v}\,\overline{x}\,d_{TV}(F,F'),
    \end{align*}

    \vspace{-8pt}
    where $d_{TV}$ denotes the total variation (TV) distance.
\end{thm}

\vspace{-5pt}
As an implication of Theorem~\ref{lem:dist_mismatch}, we can train ExPF-Net and ExS-Net with samples from distribution $F'$ and expect them to perform well under distribution $F$, provided that the mismatch between $F$ and $F'$ is not arbitrarily large. Later in Sec.~\ref{sec:exp:dist_mismatch}, we will verify this result through numerical simulations.
% 
The proof of Theorem~\ref{lem:dist_mismatch} is included in Appendix~\ref{sec:dist_mismatch}.

% \textcolor{orange}{Alec: why is Theorem \ref{lem:dist_mismatch} different from prior art? what results in the literature are most similar to it, and how does it relax assumptions/extend prior work?}
% The result guarantees that a mechanism trained under one distribution will work well under a slightly shifted distribution during inference. 



%\textcolor{blue}{we can skip the definition following this.. and include in appedix page 1?.. or maybe skip it entirely as it is well-known} between two probability distributions, i.e. given distributions $F_1$, $F_2$ over space $\Xcal$, their TV distance is defined as
%    \[d_{TV}(F_1,F_2)=\sup _{g: \mathcal{X} \rightarrow[-1,1]}\Big|\int g d F_1-\int g d F_2\Big|.\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Compared to the egalitarian notion that aims to maximize the utility of the least satisfied agent irrespective of the inefficiency and the utilitarian notion of welfare that maximizes efficiency while disregarding the fairness, NSW sits in-between \cite{kaneko1979nash,bertsimas2011price} and achieves a good trade-off between fairness and efficiency. 

    \item Designing national policies for the allocation of deceased donor kidneys/ organs in general to patients on a waiting list, in a fair and efficient way while ensuring that the donor agencies are transparent about the history of the patients is an important application that falls under this framework.

\cite{GuoContizer} consider the problem of dividing multiple divisible goods between $2$ agents and show that any IC mechanism achieves at most $0.841$ of the optimal social welfare in the worst case. 

More recently~\cite{ivanov2022optimal} extend to situations where `equivariance' is desired by replacing the feed-forward NN with Transformers. 

Resource allocation studies how to allocate resources to  participating agents holding private preferences  with the goal of maximizing a collective criterion such as cumulative revenue \cite{manelli2007multidimensional} or social welfare \cite{balseiro2019multiagent,padala2021mechanism}, while ensuring  incentive compatibility~\cite{hurwicz1973design}.

Applications appear across diverse domains such as allocation of computing budget~\cite{BGGJ22}, industrial procurement~\cite{GRJRNC04}, equitable food allocation by food banks~\cite{Pre17}, inventory allocation in  retail~\cite{Caro2010ZaraUO}, and matters of estate planning~\cite{BT96,Mou04}.

The optimal mechanism trained to optimize the sample-averaged metrics in \eqref{eq:ExPF_obj_ERM} approaches the solution of \eqref{eq:ExPF-Net_train_obj} as the number of collected samples increases -- the gap between them is known as the \textbf{generalization error} \cite{SSB14}. In Section~\ref{sec:generalization_bounds}, we provide an explicit finite-sample bound on the generalization error for the proposed ExS-Net mechanism.

==> wsc24style.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% File contains:
%   fancyhdr.sty
%   psfig.sty
%   url.sty
%   wsc.bst
%   wscpaperproc.cls
%   wscsetup.sty
%   wsc.sty
%   wscbib.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



